Long-term Monitoring of Kernel and Hardware Events to Understand Latency Variance

This paper presents our experience to understand latency variance caused by kernel and hardware events, which are often invisible at the application level. For this purpose, we have built VarMRI, a tool chain to monitor and analyze those events in the long term. To mitigate the "big data" problem caused by long-term monitoring, VarMRI selectively records a subset of events following two principles: it only records events that are affecting the requests recorded by the application; it records coarse-grained information first and records additional information only when necessary. Furthermore, VarMRI introduces an analysis method that is efficient on large amount of data, robust on different data set and against missing data, and informative to the user. VarMRI has helped us to carry out a 3,000-hour study of six applications and benchmarks on CloudLab. It reveals a wide variety of events causing latency variance, including interrupt preemption, Java GC, pipeline stall, NUMA balancing etc.; simple optimization or tuning can reduce tail latencies by up to 31%. Furthermore, the impacts of some of these events vary significantly across different experiments, which confirms the necessity of long-term monitoring.

==> pseudo_interrupts.tex <==
struct stack_per_core{
    time_t start_time[MAX_DEPTH];
    long preempted_length[MAX_DEPTH];
    int level;
}shadow_stack[MAX_CPU_ID];

begin_interrupt_fault(cpu_id, interrupt_type)
    stack = shadow_stack[cpu_id];
    stack.start_time[stack.level] = time();
    stack.preempted_length[stack.level] = 0;
    stack.level++;

end_interrupt_fault(cpu_id, interrupt_type)
    stack = shadow_stack[cpu_id];
    stack.level --;
    total_len = time() - stack.start_time[stack.level];
    actual_len = total_len - stack.preempted_length[stack.level];
    if(stack.level > 0)
       stack.preempted_length[stack.level-1]+=total_len;
    add actual_length to TCM;
     

